Transcending Adversarial Perturbations: Manifold-Aided Adversarial Examples with Legitimate Semantics

Deep neural networks were significantly vulnerable to adversarial examples manipulated by malicious tiny perturbations. Although most conventional adversarial attacks ensured the visual imperceptibility between adversarial examples and corresponding raw images by minimizing their geometric distance, these constraints on geometric distance led to limited attack transferability, inferior visual quality, and human-imperceptible interpretability. In this paper, we proposed a supervised semantic-transformation generative model to generate adversarial examples with real and legitimate semantics, wherein an unrestricted adversarial manifold containing continuous semantic variations was constructed for the first time to realize a legitimate transition from non-adversarial examples to adversarial ones. Comprehensive experiments on MNIST and industrial defect datasets showed that our adversarial examples not only exhibited better visual quality but also achieved superior attack transferability and more effective explanations for model vulnerabilities, indicating their great potential as generic adversarial examples. The code and pre-trained models were available at https://github.com/shuaili1027/MAELS.git.

==> Ours/alg/alg2.tex <==
\begin{small}
\floatname{algorithm}{Algorithm}
\begin{algorithm}[h]
\setlength{\tabcolsep}{0.5cm}
\renewcommand{\arraystretch}{0.75}
\caption{Constructing a transition}
\label{alg2}
\begin{algorithmic}[1]
\small
\REQUIRE{
$S$, the training dataset. $x$, the raw image, $y$, the ground truth label corresponding to the $x$. $\theta_E$, the parameters of the $E$ network. The $\theta _G$, $\theta _D$, and $\theta _Q$ networks are pre-trained by the first stage. $F$ is the well-trained deep learning model on the $S$.
}
\WHILE{Starting the second training stage}
\FOR{$(x,y)$ in the training dataset $S$}
\STATE{Sampling $z_1 \sim N(0,I)$ and $z_3 \sim U(a,b)$}\;
\STATE{Encoding $y$ into a one-hot form ${z_2}$}\;
\STATE{$x^* = G(x|E(z_1|x),z_2,z_3)$}\;
\STATE{$x^{**} = G(x|E(z_1|x),Q(z_2|x),Q(z_3|x))$}\;
\STATE{${\theta _Q} \overset{+}{\leftarrow} {\nabla _{{\theta _Q}}}(CE(Q({z_2}|x),{z_2}))$}\;
\STATE{${\theta _D} \overset{+}{\leftarrow} {\nabla _{{\theta _D}}}( {\cal L}_{2_{th}}^{D}) $}\;
\STATE{${\theta _E} \leftarrow {\nabla _{{\theta _E}}}({\cal L}_{2_{th}}^{E}) $}\;
\STATE{${\theta _G} \overset{+}{\leftarrow} {\nabla _{{\theta _G}}}({\cal L}_{2_{th}}^{G})$}\;
\STATE{${\theta _Q} \overset{+}{\leftarrow} {\nabla _{{\theta _Q}}}({\cal L}_{2_{th}}^{Q})$}\;
\ENDFOR
\ENDWHILE
\end{algorithmic}
\end{algorithm}
\end{small}

==> Ours/alg/alg3.tex <==
\begin{small}
\floatname{algorithm}{Algorithm}
\begin{algorithm}[h]
\setlength{\tabcolsep}{0.5cm}
\renewcommand{\arraystretch}{0.75}
\caption{Searching an attacker}
\label{alg3}
\begin{algorithmic}[1]
\small
\REQUIRE{
$S$, the training dataset. $x$, the raw image, $y$, the ground truth label corresponding to the $x$. $\theta_E$, the parameters of the $E$ network. The $\theta _G$, $\theta _D$, and $\theta _Q$ networks are pre-trained by the first stage. $F$ is the well-trained deep learning model on the $S$.
}
\FOR{$(x,y)$ in the training dataset $S$}
\STATE{$z_1=E(z_1|x)$and $z_3=Q(z_3|x)$}\;
\STATE{Encoding $y$ into a one-hot form ${z_2}$}\;
\STATE{Generating a local manifold $M$ into a one-hot form ${z_2}$}\;
\FOR{$(x,y)$ in the training dataset $S$}
\ENDFOR
\IF{}
\ENDIF

\STATE{Sampling $z_1 \sim N(0,I)$ and $z_3 \sim U(a,b)$}\;
\STATE{Encoding $y$ into a one-hot form ${z_2}$}\;
\STATE{$x^* = G(x|E(z_1|x),z2,z3)$}\;
\STATE{$x^{**} = G(x|E(z_1|x),Q(z_2|x),Q(z_3|x))$}\;
\STATE{${\theta _Q} \overset{+}{\leftarrow} {\nabla _{{\theta _Q}}}(CE(Q({z_2}|x),{z_2}))$}\;
\STATE{${\theta _D} \overset{+}{\leftarrow} {\nabla _{{\theta _D}}}( L_{{\rm{c}}ritic}^{D'}) $}\;
\STATE{${\theta _E} \leftarrow {\nabla _{{\theta _E}}}(L_{critic}^{E'}) $}\;
\STATE{${\theta _G} \overset{+}{\leftarrow} {\nabla _{{\theta _G}}}(L_{{\rm{c}}ritic}^{G'})$}\;
\STATE{${\theta _Q} \overset{+}{\leftarrow} {\nabla _{{\theta _Q}}}(L_{{\rm{c}}ritic}^{Q'})$}\;
\ENDFOR
\end{algorithmic}
\end{algorithm}
\end{small}

==> Ours/fig_files/Fig-1.tex <==
\begin{figure}[!t]
    \centering  
\includegraphics[width=0.50\textwidth]{Ours/figures/FIg-1.pdf} 
\vspace{-1.0cm}
    \caption{Reconstructed examples ($x^R$) and continuous semantic variations ($x_{1 \to 6}^{SO}$) in the first testing stage. Confidence scores for predictions by MobileNet-V2 are provided for each example. Top to bottom, the two rows consist of a handwritten digit $9$ from MNIST and a scratch defect from DEFECT.} 
    \label{Fig-1}
\end{figure}

==> Ours/fig_files/figure-3.tex <==
\begin{figure*}[!ht]
    \centering  
    \includegraphics[width=1.0\textwidth]{Ours/figures/figure-3.pdf}    
    \caption{T} 
    \label{fig-3}
\end{figure*}

==> Ours/fig_files/figure-4.tex <==
\begin{figure*}[!ht]
  \centering
  \subfloat[Object1]{
    \includegraphics[width=0.9\textwidth]{Ours/figures/figure4-1.pdf}
    \label{fig:subfig1}
  }
  \vspace{-0.5mm}
  
  \subfloat[Object2]{
    \includegraphics[width=0.9\textwidth]{Ours/figures/figure4-2.pdf}
    \label{fig:subfig2}
  }\vspace{-0.5mm}
  
  \subfloat[Object3]{
    \includegraphics[width=0.9\textwidth]{Ours/figures/figure4-3.pdf}
    \label{fig:subfig3}
  }\vspace{-0.5mm}
  
  \subfloat[Object4]{
    \includegraphics[width=0.9\textwidth]{Ours/figures/figure4-4.pdf}
    \label{fig:subfig4}
  }
  
  \caption{I}
  \label{fig-4}
\end{figure*}

==> Ours/tables/table1.tex <==
\begin{table*}[!h]
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.1}
\caption{ Comparison Results of Attack Success Rate and Transferability under different methods. The victim target used is MobileNet-V2, and adversarial examples were generated for evaluation. The success rates of various attack methods were tested using these examples. Additionally, the attack transferability of these adversarial examples from MobileNet-V2 to ResNet-18 and ResNeXt-50 transfer targets was assessed. The parameters $\ell_p$ and $\Delta$ represent the parameters required for creating the attacks.}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|cl}
\hline
\hline
\specialrule{1pt}{0pt}{1pt}
\footnotesize
&
& 
\multicolumn{3}{c|}{\textbf{MNIST}}
&
&      
\multicolumn{4}{c}{\textbf{DEFECT}} 
\\ \hline
\begin{tabular}[c]{@{}c@{}}\textbf{Competitors}\\\end{tabular}& \begin{tabular}[c]{@{}c@{}} \textbf{Parameters} \\($\ell_p$, $\Delta$)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} \textbf{Victim Target*} \\ MobileNet-V2\end{tabular}   
& \begin{tabular}[c]{@{}c@{}} \textbf{Transfer Target*} \\ ResNet-18\end{tabular}               
& \begin{tabular}[c]{@{}c@{}} \textbf{Transfer Target**} \\ResNext-50\end{tabular}              
& \begin{tabular}[c]{@{}c@{}} \textbf{Parameters} \\($\ell_p$, $\Delta$)\end{tabular}                                                                   
& \begin{tabular}[c]{@{}c@{}} \textbf{Victim Target*}\\ MobileNet-V2\end{tabular}   
& \begin{tabular}[c]{@{}c@{}} \textbf{Transfer Target*}\\ ResNet-18\end{tabular}              & \begin{tabular}[c]{@{}c@{}} \textbf{Transfer Target**} \\ ResNext-50\end{tabular}              
&  \\ \hline
& ($\ell_2, \Delta=1.50$)
& 60.51\%
& 0.32\%
& 0.12\%
& 
& 
&
&
&  \\
PGD
& ($\ell_2, \Delta=3.00$)
& 87.75\%
& 0.45\%
& 0.21\%
&
& 
&
&
&  \\

& ($\ell_2, \Delta=4.50$)
&  88.31\%
&  0.70\%
&  0.21\%
&
&  
&
&
&  \\
\hline
& ($\ell_2, \Delta=1.50$)
& 59.62\%
& 0.30\%
& 0.13\%
&
&   
&
&
&  \\
PGDRS
& ($\ell_2, \Delta=3.00$)
& 60.77\%
& 0.33\%
& 0.10\%
&
& 
&
&
&  \\

& ($\ell_2, \Delta=4.50$)
& 83.91\%
& 0.45\%
& 0.14\%
&
& 
&
&
&  \\ \hline

& ($\ell_2, \Delta=4.50$)
& 9.28\%
& 0.74\%
& 0.37\% 
&
& 
&
&
&  \\
Square
& ($\ell_2, \Delta=7.50$)
& 11.93\%
& 3.41\%
& 1.46\%
&
&   
&
&
&  \\

& ($\ell_2, \Delta=12.0$)
& 13.46\%
& 7.51\%
& 4.63\%
&
&   
&
&
&  \\ \hline
& ($\ell_2, \Delta=1.50$)
&
&
&
&
&  
& 
&
&  \\
FAB
& ($\ell_2, \Delta=3.00$)
&
&
&
&
&   
&
&
&  \\

& ($\ell_2, \Delta=4.50$)
&
&
&  
&
& 
&
&
&  \\\hline
DeepFool 
&  ($\ell_2$)                                                                       
&                                                                                                                                              &  
&   &                                                                      &                                                                         &                                                                         &  \\ \hline

CW
& ($\ell_2$)                                                                        &                                                                                       &                                           &  
&
&                                                                         &                                                                         &  \\ \hline

Ours
& $/$
& 88.55\%
& 34.41\%
& 30.78\%
&
& 100.0\%
& 1.92\%
& 1.92\% \\ 
\hline
\rowcolor{gray!25}\multicolumn{10}{c}{}\\
\hline
&
& 
\multicolumn{7}{|c}{\textbf{CIFAR10}}\\\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Competitors}\\\end{tabular}& \begin{tabular}[c]{@{}c@{}} \textbf{Parameters} \\($\ell_p$, $\Delta$)\end{tabular}
& \multicolumn{3}{|c}{\begin{tabular}[c]{@{}c@{}} \textbf{Victim Target*} \\ MobileNet-V2\end{tabular}}   
& \multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}} \textbf{Transfer Target*} \\ ResNet-18\end{tabular}}               
& \multicolumn{2}{|c}{ \begin{tabular}[c]{@{}cc@{}} \textbf{Transfer Target**} \\ResNext-50\end{tabular}}                           
&  \\ \hline
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\
PGD
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\

& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\\hline
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\
PGDRS
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\

& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\\hline

& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\
Square
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\

& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\\hline
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\
FAB
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\

& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\\hline
DeepFool 
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\\hline

CW
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\\hline

Ours
& ($\ell_2, \Delta=1.50$)
& \multicolumn{3}{|c}{}
& \multicolumn{2}{|c|}{}
& \multicolumn{2}{|c}{}
&   \\
\hline
\hline
\specialrule{1pt}{0pt}{1pt}
\end{tabular}
\label{tab1}
\end{table*}

==> Ours/tables/table2.tex <==
\begin{table*}[!h]
\centering
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.05}
\caption{The strength of various attacks on two defense methods, Adversarial Training and Network Distillation. AT-MODEL represented the MODEL with a defense of Adversarial Training and ND-MODEL represented the MODEL with the defense of Network Distillation.}
\begin{tabular}{l|c|ccc|ccc}
\hline
\hline
\specialrule{1pt}{0pt}{1pt}
& & \multicolumn{6}{|c}{\textbf{MNIST}}                                                           
\\ \cline{3-8}
\textbf{Competitors}& \textbf{Parameters}
& \multicolumn{3}{c|}{\textbf{Adversarial Training}} 
& \multicolumn{3}{c}{\textbf{Network Distillation}} 
\\
& ($\ell_p$, $\Delta$)
& AT-Victim   
& AT-Transfer1   
& \multicolumn{1}{c|}{AT-Transfer2}   
& ND-Victim   
& ND-Transfer1   
& ND-Transfer2   
\\ \hline
     
& ($\ell_2$,$\Delta=1.50$)
& 0.44\%
& 0.25\%           
& 0.07\%            
&               
&            
&             
\\
PGD      
& ($\ell_2$,$\Delta=3.00$)
& 0.69\%
& 0.04\%          
& 0.15\%           
&               
&            
&             
\\     
& ($\ell_2$,$\Delta=4.50$)
& 1.77\%
& 0.17\%            
& 0.26\%            
&               
&            
&             
\\\hline
CW       
& 
& 
&            
&             
&               
&            
&             
\\\hline

Ours     
&
& 47.18\%
& 37.94\%
& 29.34\%         
&             
&               
&                        
\\ \hline
\hline
& & \multicolumn{6}{|c}{\textbf{DEFECT}}                                                           
\\ \cline{3-8}
& \textbf{Parameters}
& \multicolumn{3}{c|}{\textbf{Adversarial Training}} 
& \multicolumn{3}{c}{\textbf{Network Distillation}} 
\\
& ($\ell_p$, $\Delta$)
& AT-Victim   
& AT-Transfer1   
& AT-Transfer2   
& ND-Victim   
& ND-Transfer1   
& ND-Transfer2   
\\ \hline
     
& ($\ell_2$,$\Delta=1.50$)
& 
&            
&             
&               
&            
&             
\\
PGD      
& ($\ell_2$,$\Delta=3.00$)
& 
&            
&             
&               
&            
&             
\\     
& ($\ell_2$,$\Delta=4.50$)
& 
&            
&             
&               
&            
&             
\\\hline
CW       
& 
& 
&            
&             
&               
&            
&             
\\\hline

Ours     
&
& 
&            
&             
&               
&            
&             
\\  
\hline
\hline
& & \multicolumn{6}{|c}{\textbf{CIFAR10}}  
\\  \cline{3-8}
& \textbf{Parameters}
& \multicolumn{3}{c|}{\textbf{Adversarial Training}} 
& \multicolumn{3}{c}{\textbf{Network Distillation}} 
\\
& ($\ell_p$, $\Delta$)
& AT-Victim   
& AT-Transfer1   
& AT-Transfer2   
& ND-Victim   
& ND-Transfer1   
& ND-Transfer2   
\\ \hline
     
& ($\ell_2$,$\Delta=1.50$)
& 0.44\%
& 0.25\%           
& 0.07\%            
&               
&            
&             
\\
PGD      
& ($\ell_2$,$\Delta=3.00$)
& 0.69\%
& 0.04\%          
& 0.15\%           
&               
&            
&             
\\     
& ($\ell_2$,$\Delta=4.50$)
& 1.77\%
& 0.17\%            
& 0.26\%            
&               
&            
&             
\\\hline
CW       
& 
& 
&            
&             
&               
&            
&             
\\\hline

Ours     
&
& 47.18\%
& 37.94\%
& 29.34\%         
&             
&               
&                        
\\ \hline
\hline
\specialrule{1pt}{0pt}{1pt}

\end{tabular}
\label{tab2}
\end{table*}

==> Ours/tables/table3.tex <==
\begin{table}[!h]
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.1}
\caption{Results of Ps and Cs. For several sets shown in Fig. \ref{fig-4}, we gave results of corresponding prediction metrics for each set under three models. Taking Object1 as an example, the order ($Raw\to Ord_1\to Ord_2\to Ord_3\to Ord_4$ ) represented a series of continuously generated exam0ples under our method. By controlling the change of a certain dimension, the target semantics in raw images change continuously. In this process, the nature of the generated examples also changes from non-adversarial (green-marked orders) to adversarial (red-marked orders). }
\centering
\begin{tabular}{|c|c|c|ccccc|}
\hline
\hline
\specialrule{1pt}{0pt}{1pt}
&                               
&                           
& \multicolumn{5}{c|}{Our Generated Examples}                                             \\ \cline{4-8}

\multirow{-2}{*}{Raw images}                                                    
& \multirow{-2}{*}{Models}      
& \multirow{-2}{*}{Metrics} 
& $Raw$                            
& $Ord_1$                                       
& $Ord_2$                                     
& $Ord_3$                                     
& $Ord_4$                                     
\\ 
\hline
\hline

&                               
& P           
& {\color[HTML]{009901} \textbf{1}}     
& {\color[HTML]{009901} \textbf{1}}       
& {\color[HTML]{009901} \textbf{1}}       
& {\color[HTML]{009901} \textbf{1}}       
& {\color[HTML]{009901} \textbf{1}}                  
\\

& \multirow{-2}{*}{Victim} 
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}    
\\ \cline{2-8} 

&                               
& P           
& {\color[HTML]{009901} \textbf{1}}     
& {\color[HTML]{009901} \textbf{1}}       
& {\color[HTML]{009901} \textbf{1}}       
& {\color[HTML]{009901} \textbf{1}}       
& {\color[HTML]{009901} \textbf{1}}                    
\\

& \multirow{-2}{*}{Transfer1}    
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}        
\\ \cline{2-8} 

&                               
& P           
& {\color[HTML]{009901} \textbf{1}}     
& {\color[HTML]{009901} \textbf{1}}       
& {\color[HTML]{009901} \textbf{1}}       
& {\color[HTML]{009901} \textbf{1}}       
& {\color[HTML]{009901} \textbf{1}}                    
\\

\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Object1\\ \\ (MNIST)\end{tabular}}  
& \multirow{-2}{*}{Transfer2}   
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}      
\\ 
\hline
\hline

&
& P           
&{\color[HTML]{009901} \textbf{5}}     
& {\color[HTML]{009901} \textbf{5}}       
& {\color[HTML]{009901} \textbf{5}}       
& {\color[HTML]{009901} \textbf{5}}       
& {\color[HTML]{009901} \textbf{5}}                  
\\

& \multirow{-2}{*}{Victim} 
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
 \\ \cline{2-8} 

&                               
& P           
& {\color[HTML]{009901} \textbf{5}}     
& {\color[HTML]{009901} \textbf{5}}       
& {\color[HTML]{009901} \textbf{5}}       
& {\color[HTML]{009901} \textbf{5}}       
& {\color[HTML]{009901} \textbf{5}}                   
\\

& \multirow{-2}{*}{Transfer1}    
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{99.99\%}} 
& {\color[HTML]{009901} \textbf{99.99\%}} 
 \\ \cline{2-8} 

&                               
& P           
& {\color[HTML]{009901} \textbf{5}}     
& {\color[HTML]{009901} \textbf{5}}       
& {\color[HTML]{009901} \textbf{5}}       
& {\color[HTML]{009901} \textbf{5}}       
& {\color[HTML]{009901} \textbf{5}}                    
\\

\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Object2\\ \\ (DEFECT)\end{tabular}} 
& \multirow{-2}{*}{Transfer2}   
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{99.99\%}} 
& {\color[HTML]{009901} \textbf{99.99\%}} 
& {\color[HTML]{009901} \textbf{99.99\%}} 
& {\color[HTML]{009901} \textbf{99.97\%}}  
\\ 
\hline
\hline

&                               
& P           
& {\color[HTML]{009901} \textbf{3}}     
& {\color[HTML]{009901} \textbf{3}}       
& {\color[HTML]{CB0000} \textbf{7}}       
& {\color[HTML]{CB0000} \textbf{7}}       
& {\color[HTML]{CB0000} \textbf{7}}                   
\\

& \multirow{-2}{*}{Victim} 
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{55.00\%}} 
& {\color[HTML]{CB0000} \textbf{76.00\%}} 
& {\color[HTML]{CB0000} \textbf{97.00\%}} 
& {\color[HTML]{CB0000} \textbf{99.00\%}}      
\\ \cline{2-8} 

&                               
& P           
& {\color[HTML]{009901} \textbf{3}}     
& {\color[HTML]{009901} \textbf{3}}       
& {\color[HTML]{009901} \textbf{3}}       
& {\color[HTML]{009901} \textbf{3}}       
& {\color[HTML]{009901} \textbf{3}}                    
\\

& \multirow{-2}{*}{Transfer1}    
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{97.00\%}}   
\\ \cline{2-8} 
                                                                                
&                               
& P          
& {\color[HTML]{009901} \textbf{3}}     
& {\color[HTML]{009901} \textbf{3}}       
& {\color[HTML]{009901} \textbf{3}}       
& {\color[HTML]{009901} \textbf{3}}       
& {\color[HTML]{009901} \textbf{3}}                  
\\

\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Object3\\ \\ (MNIST)\end{tabular}}  
& \multirow{-2}{*}{Transfer2}   
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{99.99\%}} 
& {\color[HTML]{009901} \textbf{99.98\%}} 
& {\color[HTML]{009901} \textbf{99.98\%}} 
& {\color[HTML]{009901} \textbf{99.95\%}} 
\\ 
\hline
\hline

&                               
& P           
& {\color[HTML]{009901} \textbf{4}}     
& {\color[HTML]{009901} \textbf{4}}       
& {\color[HTML]{009901} \textbf{4}}       
& {\color[HTML]{009901} \textbf{4}}       
& {\color[HTML]{009901} \textbf{4}}                    
\\

& \multirow{-2}{*}{Victim} 
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
\\ \cline{2-8} 

&                               
&P           
& {\color[HTML]{009901} \textbf{4}}     
& {\color[HTML]{009901} \textbf{4}}       
& {\color[HTML]{009901} \textbf{4}}       
& {\color[HTML]{009901} \textbf{4}}       
& {\color[HTML]{009901} \textbf{4}}                  
\\

& \multirow{-2}{*}{Transfer1}    
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}    
\\ \cline{2-8} 
                                                                                
&                               
& P           
& {\color[HTML]{009901} \textbf{4}}     
& {\color[HTML]{009901} \textbf{4}}       
& {\color[HTML]{009901} \textbf{4}}       
& {\color[HTML]{009901} \textbf{4}}       
& {\color[HTML]{009901} \textbf{4}}                  
\\

\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Object4\\ \\ (DEFECT)\end{tabular}} 
& \multirow{-2}{*}{Transfer2}   
& C                
& {\color[HTML]{009901} \textbf{100\%}} 
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
& {\color[HTML]{009901} \textbf{100\%}}   
\\ 
\hline
\hline
\specialrule{1pt}{0pt}{1pt}
\end{tabular}
\label{tab-3}
\end{table}

==> Ours/tables/table4.tex <==
\begin{table}[!h]
\setlength{\tabcolsep}{12pt}
\renewcommand{\arraystretch}{1.1}
\caption{Reconstruction accuracy under our method.}
\centering
\begin{tabular}{cccc}
\hline
\specialrule{0.5pt}{0pt}{0.5pt}
\multicolumn{4}{c}{\textbf{Reconstruction Accuracy}} 
\\\hline
Dataset
& MobileNet-V2
& ResNet-18           
& ResNeXt-50 \\ \hline

MNIST
& 99.33\%
& 99.45\%           
& 99.44\% \\ 

DEFECT
& 98.96\%
& 99.56\%           
& 99.48\% \\ 

CIFAR10
& 88.10\%
& 84.27\%           
& 90.44\%\\ 
\hline
\hline
\specialrule{0.5pt}{0pt}{0.5pt}
\end{tabular}
\label{tab-4}
\end{table}

==> Ours/tables/table5.1.tex <==
\begin{table}[!ht]
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.00}
\caption{Reconstruction accuracy of various models for raw images. Reconstruction accuracy refers to the correct accuracy of the raw and reconstructed images predicted by the target model at the same time. Reconstruction Quality shows the visual quality of the reconstructed relative raw data. \textbf{Raw}, \textbf{RECON}, and \textbf{DIFF} represent raw images, reconstructed images, and the difference between raw images and reconstructed images respectively.}
\centering
\small
\begin{tabular}{cccc}
\hline
\specialrule{1pt}{0pt}{1pt}
\multicolumn{4}{c}{\textbf{Reconstruction Accuracy}} 
\\\hline

Dataset
& MobileNet-V2
& ResNet-18  
& ResNeXt-50 \\ \hline

MNIST
& 99.33\%
& 99.45\%   
& 99.44\% \\ 

DEFECT
& 98.96\%
& 99.56\%  
& 99.48\% \\ 
\hline
\hline
\specialrule{1pt}{0pt}{1pt}
\multicolumn{4}{c}{\textbf{Reconstruction Quality}} 
\\\hline
\multicolumn{4}{c}{\includegraphics[width=0.50\textwidth]{Ours/figures/ReconstructionComparsion.pdf}}
 \\ \hline
\hline
\specialrule{1pt}{0pt}{1pt}
\end{tabular}
\label{tab-reconstructions}
\end{table}

==> Ours/tables/table5.tex <==
\begin{table*}[!t]
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\caption{Reconstruction accuracy of various models for raw images. Reconstruction accuracy refers to the correct accuracy of the raw and reconstructed images predicted by the target model at the same time. Reconstruction Quality shows the visual quality of the reconstructed relative raw data. \textbf{Raw}, \textbf{RECON}, and \textbf{DIFF} represent raw images, reconstructed images, and the difference between raw images and reconstructed images respectively.}
\centering
\begin{tabular}{cccccccccccccccccccc}
\hline
\specialrule{1pt}{0pt}{1pt}
\multicolumn{20}{c}{\textbf{Reconstruction Accuracy}} 
\\\hline

&&&&&&&&&&&
& Dataset
&
& MobileNet-V2
&
& \multicolumn{1}{c}{ResNet-18}   
&
& ResNeXt-50 \\ \hline

&&&&&&&&&&&
&MNIST
&
& \multicolumn{1}{c}{99.33\%}
&
& 99.45\%   
&
& 99.44\% \\ 

&&&&&&&&&&&
&DEFECT
&
& 98.96\%
&
& 99.56\%  
&
& 99.48\% \\ 

&&&&&&&&&&&
&CIFAR10
&
& 88.10\%
&
& 84.27\% 
&
& 90.44\%\\ 
\hline
\hline
\specialrule{1pt}{0pt}{1pt}
\multicolumn{20}{c}{\textbf{Reconstruction Quality}} 
\\\hline
\multicolumn{20}{c}{\includegraphics[width=0.95\textwidth]{Ours/figures/recon.pdf}}
 \\ \hline
\hline
\specialrule{1pt}{0pt}{1pt}
\end{tabular}
\label{tab-reconstructions}
\end{table*}
